Logarithmic Regret from Sublinear Hints

We consider the online linear optimization problem, where at every step the algorithm plays a point $x_t$ in the unit ball, and suffers loss $\langle c_t, x_t\rangle$ for some cost vector $c_t$ that is then revealed to the algorithm. Recent work showed that if an algorithm receives a hint $h_t$ that has non-trivial correlation with $c_t$ before it plays $x_t$, then it can achieve a regret guarantee of $O(\log T)$, improving on the bound of $\Theta(\sqrt{T})$ in the standard setting. In this work, we study the question of whether an algorithm really requires a hint at every time step. Somewhat surprisingly, we show that an algorithm can obtain $O(\log T)$ regret with just $O(\sqrt{T})$ hints under a natural query model; in contrast, we also show that $o(\sqrt{T})$ hints cannot guarantee better than $\Omega(\sqrt{T})$ regret. We give two applications of our result, to the well-studied setting of optimistic regret bounds and to the problem of online learning with abstention.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec:prelim}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Missing proofs are in the Appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> direct.tex <==
\section{Possible direct algorithm}

\newcommand{\ball}{\mathcal{B}_2^d}

We start with the following mild variant of the FTRL lemma:

\begin{lemma}
Suppose $\psi_0, \psi_1, \dots$ are functions $\mathbb{R}^d \mapsto \mathbb{R}$, such that $\psi_0 (x) = r_0 \norm{x}^2$, and $\psi_t (x) = \iprod{c_t, x} + r_t \norm{x}^2$. Define
\[ x_{t+1} = \argmin_{x \in \ball} ~\psi_{0:t} (x). \]
Then for any $u \in \ball$, we have
\[ \sum_{t=1}^T \iprod{c_t, x_t} - \iprod{c_t, u} \le r_0 \norm{u}^2 + \sum_{t=1}^T r_t \left(  \norm{u}^2 - \norm{x_{t+1}}^2 \right) + \sum_{t=1}^T \iprod{c_t, x_t - x_{t+1}}. \]
\end{lemma}
\begin{proof}
We will first show that
\[ \sum_{t=1}^T \psi_t (x_t) - \psi_t (u) \le [ \psi_0 (u) - \psi_0 (x_1) ] + \sum_{t=1}^T \psi_t (x_t) - \psi_t (x_{t+1}). \]
The above inequality rearranges to
\[ \sum_{t=0}^T \psi_t (x_{t+1}) \le \sum_{t=0}^T \psi_t (u).  \]
This can be shown by induction, as in the standard proof of the FTL lemma.  Now, plugging in the expression for $\psi_t$, and using $x_1 = 0$, the conclusion of the lemma follows.
\end{proof}

The new algorithm can be described as follows.  It assumes that the cost vectors are $\Theta(1)$ in length, and that $\alpha$ is known.  Let us define 
\[ R_t = \sqrt{t},~~~ r_t = R_t - R_{t-1}, ~~~ x_{t+1} = \argmin_{x \in \ball} \iprod{G_t, x} + R_t \norm{x}^2, \]
where $G_t = c_{1:t}$.  The algorithm is then:

\begin{enumerate}
\item at each time $t$, compute $x_t$
\item if $\norm{x_t} \le 1/2$, then define $p_t = \frac{10}{\alpha \sqrt{t}}$ and
\[ x_t' = \begin{cases} x_t - \frac{h_t}{2} \text{ with probability } p_t, \\ x_t \text{ otherwise.} \end{cases} \]
\item otherwise, define $p_t = \frac{16}{\alpha} \cdot \frac{1}{\norm{x_t} \norm{G_{t-1}}} $, and 
\[ x_t' = \begin{cases} -h_t \text{ with probability } p_t, \\ x_t \text{ otherwise.} \end{cases} \]
\item ask for $h_t$ with probability $p_t$ as above, and play the point $x_t'$
\end{enumerate}

In the first case, since $\norm{h_t} \le 1$, the played point has norm $\le 1$.  Before beginning the analysis, note that the global minimizer of $\iprod{G_t, x} + R_t \norm{x}^2$ is $- \frac{G_t}{2R_t}$.  If this point has norm $< 1$, it will itself be $x_{t+1}$. Else, we will have $x_{t+1} = - \frac{G_t}{\norm{G_t}}$. This observation leads to the following lemma.

\begin{lemma}\label{lem:iterate-difference}
For any two successive iterations, we have
\[ \norm{x_t - x_{t+1}} \le 4 \cdot \min \left\{ \frac{1}{R_t}, \frac{1}{\norm{G_t}} \right\}. \]
\end{lemma}
\begin{proof}
The proof proceeds by considering two cases, and uses the structure of the optimum point $x_t$ described above.
\end{proof}

The regret analysis will now proceed separately for the two cases in the algorithm.  

\begin{lemma}\label{lem:case1}
Consider a time step $t$ in which $\norm{x_t} \le 1/2$.  Then we have
\[ \E[\iprod{c_t, x_t'}] \le  \iprod{c_t, x_t} - r_t - \norm{x_{t+1} - x_t}.   \]
\end{lemma}
\begin{proof}
From the definition of $x_t'$, we have that
\[ \E[ \iprod{c_t, x_t'}] = \iprod{c_t, x_t} - \frac{p_t}{2} \iprod{c_t, h_t} \le \iprod{c_t, x_t} - \frac{5}{\sqrt{t}},  \]
since we assumed that whenever a hint is obtained, $\iprod{c_t, h_t} \ge \alpha$. Next, using Lemma~\ref{lem:iterate-difference} along with the value of $r_t$, the conclusion follows.
\end{proof}

\begin{lemma}\label{lem:case2}
Let $t$ be a time step with $\norm{x_t} \ge 1/2$, and let $u \in \ball$ be any vector. We have
\[ \E[ \iprod{c_t, x_t'} ] \le \iprod{c_t, x_t} + \frac{4}{\alpha} \int_{\norm{G_{t-1}}^2}^{\norm{G_t}^2} \frac{dz}{z} - r_t (\norm{u}^2 - \norm{x_{t+1}}^2) - \norm{x_{t+1} - x_t}.  \]
\end{lemma}
\begin{proof}
Note that the assumption $\norm{x_t} \ge 1/2$ is equivalent to $\norm{G_{t-1}} \ge R_{t-1}$, because of our earlier observation about the closed form for $x_t$. 

Now, the key observation is that the second term (involving $r_t$) in the desired bound can essentially be ignored.  This is because of the following: if $G_t \ge 2 R_t$, then we have that $\norm{x_{t+1}} =1$, and thus $r_t (\norm{u}^2 - \norm{x_{t+1}}^2) \le 0$.  If not, then because we are in the case of $\norm{G_{t-1}} \ge R_{t-1}$, we will also have $G_t \ge R_t/2$, and thus $\norm{G_t} = \Theta(R_t)$.  In this case, the (bound on the) third term will be the same order as the second one, and thus it suffices to obtain the bound with a slightly higher coefficient for the third term.  (**Needs more details.**)  

Thus in what follows, we will prove that 
\[ \E[ \iprod{c_t, x_t'} ] \le \iprod{c_t, x_t} +  \frac{4}{\alpha} \int_{\norm{G_{t-1}}^2}^{\norm{G_t}^2} \frac{dz}{z} - \frac{8}{\norm{G_t}}. \]
By the definition of $x_t'$, this is equivalent to showing that
\begin{equation}\label{eq:to-show2}
p_t \left( \iprod{c_t, h_t} + \iprod{c_t, x_t} \right) \ge \frac{8}{\norm{G_t}} -  \frac{4}{\alpha} \int_{\norm{G_{t-1}}^2}^{\norm{G_t}^2} \frac{dz}{z}.
\end{equation}

By the definition of $p_t$, we have that $p_t \iprod{c_t, h_t} \ge p_t \alpha \ge \frac{16}{\norm{G_{t-1}}}$.  Thus, it is $\ge \frac{8}{\norm{G_t}}$, with a slack of $\frac{8}{\norm{G_{t-1}}}$.  (**slight error**)

Let us thus focus on the second term, $p_t \iprod{c_t, x_t}$.  The high level intuition is that if this term is negative, then $\norm{G_t}$ is larger than $\norm{G_{t-1}}$, and thus it can be charged to the integral on the RHS.  To formalize this, we start by observing that by our choice of $p_t$, we have that $p_t x_t = - \frac{16}{\alpha} \cdot \frac{G_{t-1}}{\norm{G_{t-1}}^2}$.  Thus, to show~\eqref{eq:to-show2}, it suffices to have
\begin{equation}\label{eq:to-show3}
\frac{16}{\alpha \norm{G_{t-1}^2}} \iprod{c_t, G_{t-1}} \le \frac{8}{\norm{G_{t-1}}} + \frac{8}{\alpha} \int_{\norm{G_{t-1}}^2}^{\norm{G_t}^2} \frac{dz}{z}.
\end{equation}

Next, observe that
\[ G_t = G_{t-1} + c_t \implies 2 \iprod{G_{t-1}, c_t} = \norm{ G_t}^2 - \norm{G_{t-1}}^2 - \norm{c_t}^2. \]

Thus we bound the LHS of~\eqref{eq:to-show3} as
\begin{align*}
\frac{16}{\alpha \norm{G_{t-1}}^2} \iprod{c_t,  G_{t-1}} &= \frac{8}{\alpha} \cdot \frac{\norm{G_{t}}^2 - \norm{G_{t-1}}^2 - \norm{c_t}^2}{\norm{G_{t-1}}^2} \\
&\le \frac{8}{\alpha} \cdot \frac{\norm{G_t}^2 - \norm{G_{t-1}}^2}{\norm{G_{t-1}}^2}.
\end{align*}

To complete the proof, let us define $\delta = \frac{\norm{G_t}^2 - \norm{G_{t-1}}^2}{\norm{G_{t-1}}^2}$, so that
\[ \int_{\norm{G_{t-1}}^2}^{\norm{G_t}^2} \frac{dz}{z} = \log (1+\delta) \ge \delta - \delta^2, \]
for $\delta \in (-1/2, 1/2)$.  In our setting, $| \delta | = O(1/\norm{G_{t-1}})$, and thus as long as $\norm{G_{t-1}} > \frac{1}{\alpha}$, the desired conclusion holds.
\end{proof}






==> expectedhints.tex <==


\section{Hints in Expectation}

Consider the following game:
\begin{itemize}
    \item Adversary commits to cost vector $c_t$.
    \item Learner receives randomized hint $h_t$ such that $\E[\langle c_t, h_t\rangle]\ge \alpha \E[\|c_t\|^2]$ (note that this is much stronger than asking that $\E[\langle c_t, h_t\rangle]\ge \alpha \|\E[c_t]\|^2$).
    \item Learner chooses $x_t$ and suffers loss $\langle c_t, x_t\rangle$.
\end{itemize}

For example, this protocol is implemented by having $h_t$ equal to $c_t$ for an $\alpha$-fraction of the coordinates, and having $h_t$ be some mean-zero random values for the other coordinates.

Notice that the total number of ``bad hints'', when $\langle c_t, h_t\rangle <0$ could be quite large. As an example: in a 2d problem, we could have $c_t=(\pm 1, \pm 1)$ with equal probability on all 4 options, and $h_t$ has first coordinate equal to $c_t$'s first coordinate, and second coordinate randomly $\pm 2$. Then $\langle h_t,c_t\rangle= 1 \pm2 $ uniformly at random, and so is negative about half the time.

In this setting, we use a variant of the ICML algorithm, as presented in Algorithms \ref{alg:constrained-simple} and \ref{alg:sc}. A couple things have changed:
\begin{enumerate}
    \item The surrogate loss $\ell_t$ is no longer guaranteed to be convex! This is actually ok because \emph{in expectation} it is convex.
    \item The inner strong-convex learner has changed a bit, although it is probably actually simpler here.
\end{enumerate}


\begin{algorithm}[t]
   \caption{OLO with expected hints}
   \label{alg:constrained-simple}
   \begin{algorithmic}
   \STATE \textbf{Input: } Hints $h_t$ followed by cost vectors $c_t$, expected quality parameter $\alpha$.
    \FOR{$t=1\dots T$}
    	\STATE Get hint $h_t$
    	\STATE Get  $\xbar_t$ from strongly-convex learner, and set 
    	
    	\[
    	x_t = \xbar_t + \frac{(\|\xbar_t\|^2-1)}{4} h_t
    \]
	\STATE Play $x_t$ and receive cost $c_t$
	\STATE Define $\ell_t(x) = \langle c_t, x\rangle + \frac{\langle c_t, h_t\rangle}{4}(\|x\|^2-1)$.
	\STATE Set $\mu_t = \frac{\alpha}{2} \|c_t\|^2$.
	\STATE Send the loss function $\ell_t(x)$ and expected strong-convexity $\mu_t$ to strongly-convex learner.
	\ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
   \caption{strongly convex learner}
   \label{alg:sc}
   \begin{algorithmic}
   \STATE $\xbar_t = 0$.
    \FOR{$t=1\dots T$}
    	\STATE Get (possibly non-convex, but differentiable!) loss $\ell_t(x)$ and expected strong-convexity parameter $\mu_t$.
    	\STATE Set $g_t=\nabla \ell_t(\bar x_t)$.
    	\STATE Set $\xbar_{t+1} = \argmin_{\|x\|\le 1}\frac{1}{2}\|x\|^2 +\sum_{\tau=1}^t \langle g_\tau, x\rangle + \frac{\mu_\tau}{2}\|x\|^2$
    	\STATE Output $\xbar_t$.
	\ENDFOR
\end{algorithmic}
\end{algorithm}

Observe the following two important facts:
\begin{lemma}\label{lem:surrogate-properties}
$\ell_t$ satisfies:
\begin{enumerate}
\item $\ell_t (\xbar_t) = \iprod{c_t, x_t}$.
\item For all $u$ with $\norm{u} \le 1$, $\E[\ell_t (u)] \le \iprod{c_t, u}$.
\end{enumerate}
\end{lemma}
This implies:
\begin{align*}
    \E[\sum_{t=1}^T \langle c_t, x_t - u\rangle] \le \E[\sum_{t=1}^T \ell_t(\xbar_t)-\ell_t(u)]
\end{align*}
So now we need only control the expected regret of $\xbar$ with respect to $\ell_t$, which is done in the following lemma:

\begin{lemma}\label{lem:expectedlogregret}
Suppose that $\ell_t$ and $\mu_t$ are as generated in Algorithm \ref{alg:constrained-simple}, and $\E[\langle c_t, h_t\rangle|c_t]\ge \alpha \|c_t\|^2$ for all $t$. Then
\begin{align*}
    \E[\sum_{t=1}^T \ell_t(\xbar_t)-\ell_t(u)]&\le \frac{1}{2}+\frac{8}{\alpha}\log(T+1)
\end{align*}
where the expectation is taken over any potential randomness in the choices of both $h_t$ and $c_t$.
\end{lemma}
\begin{proof}
By some algebra, we have:
\begin{align*}
    \ell_t(\xbar_t)-\ell_t(u) &=\langle g_t, \xbar_t - u\rangle -\frac{\langle c_t, h_t\rangle}{4} \|\xbar - u\|^2\\
    \intertext{taking expectations over $h_t$, but not yet over $c_t$:}
    \E[\ell_t(\xbar_t) - \ell_t(u)] &\le\E[\langle g_t, \xbar_t - u\rangle] -\frac{\alpha \|c_t\|^2}{4}\|\xbar - u\|^2]\\
    &=\E[\langle g_t, \xbar_t - u\rangle] -\frac{\mu_t}{2}\|\xbar - u\|^2]\\
    \intertext{Define $\hat \ell_t(x) = \langle g_t, x\rangle + \frac{\mu_t}{2}\|x\|^2$:}
    &=\E[\hat \ell_t(x) - \hat \ell_t(u)]
\end{align*}
Now, $\xbar_t$ is given by FTRL on the losses $\hat \ell_t$ with regularizer $\frac{1}{2}\|x\|^2$ so by \cite{mcmahan2017survey} Theorem 1, we have:
\begin{align*}
    \sum_{t=1}^T \hat \ell_t(\xbar) - \hat \ell_t(u)&\le \frac{1}{2}\|u\|^2+\sum_{t=1}^T \frac{\|g_t\|^2}{2+2\sum_{\tau=1}^t\mu_\tau}
\end{align*}

Next, observe that $g_t = c_t + \frac{\langle c_t, h_t\rangle}{2} \xbar$ so that $\|g_t\|^2\le \frac{\|c_t\|^2}{4}$. Therefore, since $\mu_t=\frac{\alpha}{2}\|c_t\|^2$, we have $\mu_t\ge \frac{\alpha}{8}\|g_t\|^2$ so that:
\begin{align*}
    \sum_{t=1}^T \frac{\|g_t\|^2}{2+2\sum_{\tau=1}^t\mu_\tau}
    &\le \frac{4}{\alpha}\sum_{t=1}^T \frac{\|g_t\|^2}{1+ \sum_{\tau=1}^t\|g_\tau\|^2}\\
    &\le \frac{8}{\alpha}\log(T+1)
\end{align*}
\end{proof}


